Rank Collapse Causes Over-Smoothing and Over-Correlation in Graph Neural Networks

Our study reveals new theoretical insights into over-smoothing and feature over-correlation in graph neural networks. Specifically, we demonstrate that with increased depth, node representations become dominated by a low-dimensional subspace that depends on the aggregation function but not on the feature transformations. For all aggregation functions, the rank of the node representations collapses, resulting in over-smoothing for particular aggregation functions. Our study emphasizes the importance for future research to focus on rank collapse rather than over-smoothing. Guided by our theory, we propose a sum of Kronecker products as a beneficial property that provably prevents over-smoothing, over-correlation, and rank collapse. We empirically demonstrate the shortcomings of existing models in fitting target functions of node classification tasks.

==> chapters/complex_eigenvectors.tex <==

%As each matrix does have $n$ eigenvalues over the field of complex numbers, we will use these to form our subspaces. We also know that for each complex eigenvalue $\lambda_i\in\mathbb{C}$ with eigenvector $\mathbf{v}_i\in\mathbb{C}^{n}$, its complex conjugate $\bar{\lambda}_i\in\mathbb{C}$ is also an eigenvalue with corresponding eigenvector $\bar{\mathbf{v}}_i\in\mathbb{C}^{n}$. Further, the conjugate pairs $\mathbf{v}_i$ and $\bar{\mathbf{v}}_i$ together span a 2-dimensional subspace in $\mathbb{R}$ with basis vectors Re$(\mathbf{v}_i)\in\mathbb{R}^{n\times n}$ and Im$(\mathbf{v}_i)\in\mathbb{R}^{n\times n}$~\cite{}. 
%Therefore, we use this 2-dimensional subspace $\mathbf{V}_i\in\mathbb{R}^{n\times 2}$ in the case of complex eigenvalues and a 1-dimensional subspace $\mathbf{V}_j\in\mathbb{R}^{n\times 1}$ in the case of real eigenvalues as in the symmetric case.
%We make use of these subspaces and combine them with a full rank matrix $\mathbf{U}\in\mathbb{R}^{d\times d}$ as before. This leads to our invariant subspaces 
%\begin{equation}
%    \mathbf{S}_{(i)} = \begin{cases}
%    \mathbf{U}\otimes \mathbf{v}_i, & \mathrm{if} \, \mathbf{v}_i\in\mathbb{R}^n\\ \mathbf{U}\otimes [\mathbf{v}_i \bar{\mathbf{v}}_i], & \mathrm{otherwise}
%    \end{cases}
%\end{equation}
%offering two different cases, namely a $(2\cdot d)$-dimensional subspace for the complex eigenvalues and a $d$-dimensional subspace for the real eigenvalues.
%We further denote the space spanned by each set of basis vectors as $\mathcal{T}_i = span(\mathbf{V}_i)$ and the magnitude of the corresponding eigenvalues of $\mathbf{S}_{(i)}$ with $|\lambda^\mathbf{A}_i|$ as the eigenvalues of both $\mathbf{v}_i$ and $\bar{\mathbf{v}}_i$ have the same magnitude.

%\begin{lemma}
%    \label{pr:stoch_iter}
%    Let $\mathbf{S}_i$ be defined as above and $\psi(\mathbf{X}) = \mathbf{A}\mathbf{XW}$ using any non-negative matrix $\mathbf{A}\in\mathbb{R}^{n\times n}$ and any $\mathbf{W}\in\mathbb{R}^{d\times d}$. 
%    Then, $$\frac{L((\psi),\mathbf{S}_{(i)}))}{L((\psi), \mathbf{S}_{(1)})} 
%    \leq \frac{|\lambda_i^{\mathbf{A}}|}{\lambda_1^{\mathbf{A}}} \frac{L((),\mathbf{S}_{(i)})}{L((), \mathbf{S}_{(1)})}
%    $$
%\end{lemma}

==> chapters/decomposition.tex <==
\section{Decomposition into invariant subspaces}
\label{sec:decomp}


%1. For a given convolution, we split our state space into a subspaces, for which our state is just a linear combination of basis vectors from each subspace. We design these subspaces to be invariant to our convolution so that we can analyze the change for each subspace individually. state into a combination of vectors that are each part of a subspace that is invariant to the convolution

%2. Let us write a state X as a linear combination of some basis vectors (S \otimes Q). We first consider a linear convolution, then we can apply \psi on each basis vector individually. But we form sets of these basis vectors that together form a space that is invariant to \psi. We further analyze the change that the convolution has on the magnitude on these basis vectors.





Our goal is to better understand the dynamics in GNNs and the origin of over-smoothing. 
As we will show later, many typically employed GNNs induce invariant subspaces that demonstrate different dynamics.
To analyze the effect a graph convolutional operation $\psi$ has on these different parts of the representations, we now introduce a process to relate these dynamics.

%to analyze the effect a convolutional operation $\psi$ has on different parts of the representations. 
%Our theoretical insights show that there exist parts that are treated differently and over-smoothing directly results from the way the smooth part of the data is transformed by $\psi$. 

For that, we decompose a given vectorized feature matrix
\begin{equation}
    vec(\mathbf{X}) = \mathbf{S}\mathbf{c} = \sum_{i=1}^m \mathbf{S}_{(i)} \mathbf{c}_{(i)}
\end{equation}
into a linear combination $\mathbf{c}\in\mathbb{R}^{nd}$ of some linearly independent basis vectors $\mathbf{S}\in\mathbb{R}^{nd\times nd}$ and split these into a sum of $m$ vectors in disjoint subspaces $\mathcal{Q}_i = span(\mathbf{S}_{(i)}) \subset\mathbb{R}^{nd}$ that we will choose to be invariant to $\psi$.
This allows us to analyze the evolution of the state by considering the vector in each subspace separately. 
%We start with the general process of decomposing our state and measuring the change within each subspace.
%For a given node state $\mathbf{X}\in\mathbb{R}^{n\times d}$, we first rewrite the vectorized form 
%For that, we define two orthonormal matrices $\mathbf{Q}\in\mathbb{R}^{n\times n}$ and $\mathbf{S}\in\mathbb{R}^{d\times d}$ and make use of the Kronecker product to decompose our state 
%\begin{equation}
%    vec(\mathbf{X}) = \mathbf{S}\mathbf{c} = \sum_{i=1}^k \mathbf{S}_{(i)} \mathbf{c}_{(i)}
%\end{equation}
%as a linear combination of some linearly independent basis vectors $\mathbf{S}\in\mathbb{R}^{nd\times nd}$ with $\mathbf{c}\in\mathbb{R}^{nd}$ being the solution to $\mathbf{S} \mathbf{c} = vec(\mathbf{X})$. 
%We also split the columns $\mathbf{S}$ into $k$ sets $\mathbf{S}_{(1)},\dots,\mathbf{S}_{(k)}$ of basis vectors. 
%For each set $\mathbf{S}_{(i)}$ of vectors, we define its induced subspace as the span of its column vectors $\mathcal{T}_i = span(\mathbf{S}_{(i)})$. 
Their direct sum $\bigoplus_{i=1}^k \mathcal{Q}_i = span(\mathbf{S})$ results in the full space.
%We denote $vec(\mathbf{X})_{(i)}=\mathbf{S}_{(i)}\mathbf{c}_{(i)}$ as the part of $vec(\mathbf{X})$ in subspace $\mathcal{T}_i$.

%LINEAR LINEAR LINEAR WOHER?
As motivated before, we want to understand the linear case, for which we rewrite the state as $vec(\psi(\mathbf{X}))=\mathbf{T}vec(\mathbf{X})$ using some linear transformation $\mathbf{T}\in\mathbb{R}^{nd\times nd}$.
%split s into sets of basis vector that form a subspace of r that is invariant to the convolutional operation $\psi$.
We then use its additivity and apply $\psi$ on each subspace separately, resulting in 
\begin{equation}
%= \psi((\mathbf{S}\otimes \mathbf{Q})\mathbf{c}) 
    vec(\psi(\mathbf{X})) = \mathbf{T}vec(\mathbf{X})= \sum_{i=1}^m\mathbf{T}\mathbf{S}_{(i)}\mathbf{c}_{(i)}\, .
    % = \sum_{i\in k}\psi\left(\sum_{(l,r)\in M_i} (\mathbf{s}_l\otimes\mathbf{q}_r)c_{l,r}\right) 
\end{equation}
%For each subspace we consider how the convolution changes the magnitude of the basis \psi(A\otimes B)c we take the magnitude of $\psi(A\otimes B)$ and want to relate it to the previous state $(A\otimes B)$. For that we define a function that caluculates exactly that
We want to choose subspaces that are invariant to $\psi$, so for each $\mathcal{Q}_i$, vectors remain within $\mathcal{Q}_i$ after applying the graph convolution, i.e., $vec(\mathbf{V}) \in \mathcal{Q}_i \Rightarrow vec(\psi(\mathbf{V})) \in \mathcal{Q}_i$. We then relate the differences in the effect of $\psi$ on each of these subspaces to understand the underlying dynamics better. 

Previous work considered the effects of graph convolutions on the coefficients $\mathbf{c}$, for which coarse bounds were found~\cite{oono2019graph,cai2020note,zhou2021dirichlet}.   
We instead analyze how $\psi$ changes the basis vectors $\mathbf{S}_{(i)}$ of each subspace while keeping the coefficients $\mathbf{c}$ constant, leading to a cleaner analysis of the underlying process.
%This can be seen as understanding changes that would be put on the unit circle.
%Relating the changes in of each base will help us better understand the dynamics.

%we do not use the c when measuring the size, because it can coincidentally and ignoreing that is like putting a unit ball in each subspace and understanding how the volume changes. 

Given any node state and its decomposition into subspaces
\begin{equation}
 vec(\mathbf{X}^{(k)}) = \sum_{i=1}^m \mathbf{T}^{(k)}\dots\mathbf{T}^{(1)}\mathbf{S}_{(i)}\mathbf{c}_{(i)}\, , 
\end{equation}
we compare the magnitude of the matrices $\mathbf{S}_{(i)}$ and $\mathbf{T}^{(k)}\dots\mathbf{T}^{(1)}\mathbf{S}_{(i)}$ for each $i$ showing how much each subspace contributes to the entire state. 
%Since any $\mathbf{X}$ is expressed as an unchanged constant linear combination of transformed basis vectors, we compare the changes in basis vectors for different subspaces.
We introduce a function  
\begin{equation}
    L((\psi^{(1)},\dots,\psi^{(k)}), \mathbf{S}_{(i)}) \vcentcolon= ||\mathbf{T}^{(k)}\dots\mathbf{T}^{(1)}\mathbf{S}_{(i)}||
    %=||\mathbf{G}_{\mathcal{X}_i}^{(k)}||\cdot||\mathbf{H}_{\mathcal{Y}_i}^{(k)}||
\end{equation}
that calculates the norm of the transformed basis vectors for each subspace $\mathcal{Q}_i$, not considering the value of the coefficients $\mathbf{c}$. 

In the next section, we use this method to investigate the dynamics in various popular GNNs and show that one subspace always dominates the resulting node representations in these cases.

%show that one subspace dominates the resulting node state for many currently employed message-passing models. Typically, vectors in this subspace are similar for all nodes, resulting in over-smoothing.

==> chapters/deleted.tex <==
$$\frac{\left((\mathbf{W}^{(l)}\otimes\mathbf{A})\dots(\mathbf{W}^{(1)}\otimes\mathbf{A})(\mathbf{U}\otimes \mathbf{V})c\right)^T(\mathbf{I}_d\otimes\mathbf{\Delta})(\mathbf{W}^{(l)}\otimes\mathbf{A})\dots(\mathbf{W}^{(1)}\otimes\mathbf{A})(\mathbf{U}\otimes \mathbf{V})c}{\left((\mathbf{W}^{(l)}\otimes\mathbf{A})\dots(\mathbf{W}^{(1)}\otimes\mathbf{A})(\mathbf{U}\otimes \mathbf{V})c\right)^T(\mathbf{W}^{(l)}\otimes\mathbf{A})\dots(\mathbf{W}^{(1)}\otimes\mathbf{A})(\mathbf{U}\otimes \mathbf{V})c}\\
        &= \frac{c^T(\mathbf{U}^T\mathbf{W}^{(1)^T}\dots\mathbf{W}^{(l)^T}\otimes \mathbf{\Lambda^{\mathbf{A}}}\mathbf{V}^T)(\mathbf{I}_d\otimes\mathbf{\Delta})(\mathbf{W}^{(l)}\dots\mathbf{W}^{(1)}\mathbf{U}\otimes\mathbf{V}\mathbf{\Lambda^\mathbf{A}})c}{c(\mathbf{U}^T\mathbf{W}^{(1)^T}\dots\mathbf{W}^{(l)^T}\otimes\mathbf{\Lambda^\mathbf{A}}\mathbf{V}^T)(\mathbf{W}^{(l)}\dots\mathbf{W}^{(1)}\mathbf{U}\otimes\mathbf{V}\mathbf{\Lambda^\mathbf{A}})c}\\
        &= \frac{c(\mathbf{U}^T\mathbf{W}^{(1)^T}\dots\mathbf{W}^{(l)^T}\mathbf{W}^{(l)}\dots\mathbf{W}^{(1)}\mathbf{U}\otimes\mathbf{\Lambda^\mathbf{A}}(\mathbf{I}_n-\mathbf{\Lambda}^\mathbf{A})\mathbf{\Lambda^\mathbf{A}})c}{c(\mathbf{U}^T\mathbf{W}^{(1)^T}\dots\mathbf{W}^{(l)^T}\mathbf{W}^{(l)}\dots\mathbf{W}^{(1)}\mathbf{U}\otimes\mathbf{\Lambda^\mathbf{A}}\mathbf{\Lambda^\mathbf{A}})c}\\
        &= \frac{c(\mathbf{U}^T\mathbf{W}^{(1)^T}\dots\mathbf{W}^{(l)^T}\mathbf{W}^{(l)}\dots\mathbf{W}^{(1)}\mathbf{U}\otimes\mathbf{\Lambda^\mathbf{A}}(\mathbf{I}_n-\mathbf{\Lambda}^\mathbf{A})\mathbf{\Lambda^\mathbf{A}})c}{c(\mathbf{U}^T\mathbf{W}^{(1)^T}\dots\mathbf{W}^{(l)^T}\mathbf{W}^{(l)}\dots\mathbf{W}^{(1)}\mathbf{U}\otimes\mathbf{\Lambda^\mathbf{A}}\mathbf{\Lambda^\mathbf{A}})c}\\
        &= \frac{c(\mathbf{P}\otimes\mathbf{\Lambda^\mathbf{A}}(\mathbf{I}_n-\mathbf{\Lambda}^\mathbf{A})\mathbf{\Lambda^\mathbf{A}})c}{c(\mathbf{P}\otimes\mathbf{\Lambda^\mathbf{A}}\mathbf{\Lambda^\mathbf{A}})c}\\   
        &= \frac{c\frac{\mathbf{P}\otimes\mathbf{\Lambda^\mathbf{A}}(\mathbf{I}_n-\mathbf{\Lambda}^\mathbf{A})\mathbf{\Lambda^\mathbf{A}}}{|\lambda_1^\mathbf{P}|\cdot|\lambda_1^\mathbf{A}|}c}{c\frac{\mathbf{P}\otimes\mathbf{\Lambda^\mathbf{A}}\mathbf{\Lambda^\mathbf{A}}}{|\lambda_1^\mathbf{P}|\cdot|\lambda_1^\mathbf{A}|}c}\\ $$


\subsubsection{Proof of Lemma 4}
\begin{lemma}
    %A being any non-negative matrix
    Let $\mathbf{S}_i$ be defined as above and $\psi(\mathbf{X}) = \mathbf{A}\mathbf{XW}$ using any non-negative matrix $\mathbf{A}\in\mathbb{R}^{n\times n}$ and any $\mathbf{W}\in\mathbb{R}^{d\times d}$. 
    Then, $$\frac{L((\psi),\mathbf{S}_{(i)}))}{L((\psi), \mathbf{S}_{(1)})} 
    \leq \frac{|\lambda_i^{\mathbf{A}}|}{\lambda_1^{\mathbf{A}}} \frac{L((),\mathbf{S}_{(i)})}{L((), \mathbf{S}_{(1)})}
    $$
\end{lemma}

Proof. For subspaces $\mathbf{S}_{(i)}$ corresponding to real-valued eigenvectors $\mathbf{v}_i$ the proof is unchanged from the symmetric case. Here, we provide the proof for the complex-valued case. 
Let the matrix of eigenvalues corresponding to $\mathbf{v}_i$ and $\bar{\mathbf{v}}_i$ be $\mathbf{\Lambda}_{(i)}^\mathbf{A} = \begin{bmatrix}
\lambda_i^\mathbf{A} & 0 \\
0 & \bar{\lambda}_i^\mathbf{A}
\end{bmatrix}$.
We start by providing the following equality:

\begin{equation}
\begin{split}
    ||\mathbf{A} \begin{bmatrix}\mathbf{v}_i & \bar{\mathbf{v}}_i\end{bmatrix}||
    &= ||\begin{bmatrix}\mathbf{v}_i &\bar{\mathbf{v}}_i\end{bmatrix}\mathbf{\Lambda}_{(i)}^\mathbf{A}||\\
    &= \sqrt{\mathrm{tr}(\mathbf{\Lambda}_{(i)}^{\mathbf{A}^H}\begin{bmatrix}\mathbf{v}_i & \bar{\mathbf{v}}_i\end{bmatrix}^H\begin{bmatrix}\mathbf{v}_i & \bar{\mathbf{v}}_i\end{bmatrix}\mathbf{\Lambda}_{(i)}^\mathbf{A})}\\
    &= \sqrt{2 \lambda_i^\mathbf{A}\bar{\lambda}_i^\mathbf{A}\langle\mathbf{v}_i,\bar{\mathbf{v}}_i\rangle}\\
    &= \sqrt{2 |\lambda_i^\mathbf{A}|^2\langle\mathbf{v}_i,\bar{\mathbf{v}}_i\rangle}\\
    &= |\lambda_i^\mathbf{A}|\cdot\sqrt{2\langle\mathbf{v}_i,\bar{\mathbf{v}}_i\rangle}\\
    &= |\lambda_i^\mathbf{A}|\cdot||\begin{bmatrix}\mathbf{v}_i & \bar{\mathbf{v}}_i\end{bmatrix}||    
\end{split}
\end{equation}

Proving the Lemma now gets much easier:

\begin{equation}
    \begin{split}
        \frac{L((\psi),\mathbf{S}_{(i)})}{L((\psi), \mathbf{S}_{(1)})} 
        &= \frac{||(\mathbf{W}^{{(l)}^T}\otimes \mathbf{A})(\mathbf{U}\otimes \begin{bmatrix}\mathbf{v}_i & \bar{\mathbf{v}}_i\end{bmatrix})||}{||(\mathbf{W}^{{(l)}^T}\otimes \mathbf{A})(\mathbf{U}\otimes \mathbf{v}_1)||}\\
        &= \frac{|\lambda_i^{\mathbf{A}}|}{\lambda_1^{\mathbf{A}}}\frac{||\mathbf{W}^{{(l)}^T}\mathbf{U}\otimes \begin{bmatrix}\mathbf{v}_i & \bar{\mathbf{v}}_i\end{bmatrix}||}{||\mathbf{W}^{{(l)}^T}\mathbf{U}\otimes \mathbf{v}_1||}\\
        &= \frac{|\lambda_i^{\mathbf{A}}|}{\lambda_1^{\mathbf{A}}}\frac{||\mathbf{W}^{{(l)}^T}\mathbf{U}||\cdot ||\begin{bmatrix}\mathbf{v}_i & \bar{\mathbf{v}}_i\end{bmatrix}||}{||\mathbf{W}^{{(l)}^T}\mathbf{U}||\cdot ||\mathbf{v}_1||}\\
        &= \frac{|\lambda_i^{\mathbf{A}}|}{\lambda_1^{\mathbf{A}}}\frac{||\mathbf{U}\otimes\begin{bmatrix}\mathbf{v}_i & \bar{\mathbf{v}}_i\end{bmatrix}||}{||\mathbf{U}\otimes \mathbf{v}_1||}\\
        &= \frac{|\lambda_i^{\mathbf{A}}|}{\lambda_1^{\mathbf{A}}}\frac{L((),\mathbf{S}_{(i)})}{L((), \mathbf{S}_{(1)})}
    \end{split}
\end{equation}
\qed

==> chapters/symmetric_transformation.tex <==
\subsubsection{Symmetric Transformation}
We let $\mathbf{A}\in\mathbb{R}^{n\times n}$ be a symmetric aggregation function and start by considering a feature transformation $\mathbf{W}\in\mathbb{R}^{d\times d}$ that is also symmetric and shared across layers as proposed originally for the continuous case in~\cite{di2022graph,eliasof2021pde}. This leads to a graph convolution of the form
\begin{equation}
    vec(\mathbf{X}^{(l+1)}) = vec(\psi(\mathbf{X}^{(l)})) = vec(\mathbf{A}\mathbf{X}^{(l)}\mathbf{W}) = (\mathbf{W} \otimes \mathbf{A})vec(\mathbf{X}^{(l)})
\end{equation}
that is similar to the GCN. In the vectorized representation, we combine both matrices using the Kronecker product into a single symmetric matrix $(\mathbf{W}\otimes \mathbf{A})\in\mathbb{R}^{nd\times nd}$. Since this symmetric matrix is repeatedly applied, with the update step we perform power iteration, which is known to converge to the dominant eigenvector when normalizing the result~\cite{mises1929praktische}. 

We make use of the eigendecompositions $\mathbf{A}=\mathbf{V\Lambda^A}\mathbf{V}^T$ and $\mathbf{W} = \mathbf{U\Lambda^W} \mathbf{U}^T$.
Using further properties of the Kronecker product, we also know the eigendecomposition $\mathbf{W}\otimes \mathbf{A} = (\mathbf{U}\otimes\mathbf{V})(\mathbf{\Lambda^W}\otimes \mathbf{\Lambda^A})(\mathbf{U}\otimes\mathbf{V})^T$.


The dominant eigenvector is $\mathbf{u}_1\otimes \mathbf{v}_1$ with corresponding maximal absolute eigenvalue $\lambda_1^\mathbf{W}\lambda_1^\mathbf{A}$. Since $\mathbf{v}_1$ corresponds to the lowest frequency of the graph laplacian, the resulting node states are similar, commonly referred to as over-smoothing. The Kronecker product only results in the multiplication of $\mathbf{v}_1$ with a different scalar for each column. 

While this already shows the result of the process, we still want to describe what exactly is happening in each iteration, because our process can also be applied to the more challenging case when $\mathbf{W}$ is not guaranteed to be symmetric or different weight matrices are used in each layer, which we describe in the following sections. 

%As we are in the symmetric case, applying the graph convolution only leads to a stretching and contraction of these eigenvectors by their corresponding eigenvalue, so we define our invariant subspaces as 

We define each subspace $\mathcal{Q}_{l,r}=span(\mathbf{u}_l \otimes \mathbf{v}_r)$ as the space spanned by each eigenvector $\mathbf{u}_l\otimes \mathbf{v}_r$. When applying $\psi$, the change of the basis vectors in each subspace is just the product with its corresponding eigenvalues.

%\begin{proposition}
%    Let $\mathbf{A}\in\mathbb{R}^{n\times n}$ and $\mathbf{W}\in\mathbb{R}^{d\times d}$ be symmetric matrices. $U\otimes V$ is an orthonormal basis for $\mathbb{R}^{nd}$. For each 1-dimensional subspace $\mathcal{T}_{l,r} = span(u_l \otimes v_r)$, it follows $\forall \mathbf{v} \in \mathcal{T}_{l,r}, \mathbf{(W \otimes A)v} \in \mathcal{T}_{l,r}$.
%\end{proposition}

\begin{proposition}
    For any state $\mathbf{X}\in\mathbb{R}^{n \times d}$, let $\psi(\mathbf{X})=\mathbf{AXW}$ with $\mathbf{A},\mathbf{W}$ defined as above. Then, 
    $$L_i((\psi), (\mathbf{V}\otimes \mathbf{U})) = \lambda^\mathbf{W}_l\lambda^\mathbf{A}_r L((), (\mathbf{u}_l\otimes \mathbf{v}_r))$$
\end{proposition}

%Proof. $L(AB_{l,r}(X^{(l)})) = ||A(u_l \otimes v_r)|| = ||u_l \otimes \lambda_rv_r||= \lambda_rL(B_{l,r}(X^{(l)}))$
Depending on the spectrum of $\mathbf{W}$, multiple subspaces can grow unconstrained when they satisfy $|\lambda_l^\mathbf{W}\lambda_r^\mathbf{A}|>1$ or all subspace may shrink when $\lambda_1^\mathbf{W} < 1$. So while $\mathbf{X}^{(l)}$ may not converge to a state that is only part of a single subspace, it will always get dominated by the one subspace corresponding to both the dominant eigenvectors from $\mathbf{W}$ and $\mathbf{A}$.
We show this by normalizing the growth of each subspace by the largest subspace. For all subspaces that do not correspond to the maximum eigenvalues of both $\mathbf{A}$ and $\mathbf{W}$ the normalized norm of its basis vectors converges to $\mathbf{0}$, which we show in the following Lemma: 

%We show this by normalizing the growth of each subspace by the largest subspace in the following Lemma:

%\begin{lemma}
%    The normalized growth of each subspace is given by $$\frac{L_{l,r}(\mathbf{AX}^{(l)}\mathbf{W})}{max_{p,q}L_{p,q}(\mathbf{AX}^{(l)}\mathbf{W})} = \frac{\lambda_l^\mathbf{W}\lambda_r^\mathbf{A}}{\lambda_1^\mathbf{W}\lambda_1^\mathbf{A}}\frac{L_{l,r}(\mathbf{X}^{(l)})}{max_{p,q}L_{p,q}(\mathbf{X}^{(l)})}$$ 
%\end{lemma}

%Proof. $\frac{L((W \otimes I_n)B_{l,r}(X^{(l)}))}{max_{p,q}L((W \otimes I_n)B_{p,q}(X^{(l)}))} = \frac{||(W \otimes I_n)u_l \otimes v_r||}{{max_{p,q}L((W \otimes I_n)B_{p,q})(X^{(l)})}} = \frac{||\lambda_lu_l \otimes v_r||}{{max_{p,q}L((W \otimes I_n)B_{p,q}(X^{(l)}))}}= \frac{\lambda_l^W}{\lambda_{\max}^W}\frac{L(B_{l,r}(X^{(l)}))}{max_{p,q}L(B_{p,q}(X^{(l)}))}$

%Since all eigenvectors corresponding to $x$ are constant across one feature, the largest subspace not corresponding to constant values is $\lambda_2\lambda_1\lambda_1\lambda_1=\lambda_2\lambda_1$ so the convergence rate does not depend on $W$.
%describe case when two eigenvalues have the same value -> still constant
%which also shows that it does not converge to a constant state, as argued before because multiple subspaces can have $|\lambda_i\lambda_j| > 1$

\begin{proposition}
    Let $\mathbf{A}\in\mathbb{R}^{n\times n}$, $\mathbf{W}\in\mathbb{R}^{d\times d}$ be symmetric matrices and $\mathbf{X}^{(l+1)}=\mathbf{AX}^{(l)}\mathbf{W}$ for any initial $\mathbf{X}^{(0)}\in\mathbb{R}^{n\times d}$. Then, 
    $$\lim_{l\to\infty}\frac{L((\psi^{(l)},\dots,\psi^{(1)}), (\mathbf{u}_l\otimes \mathbf{v}_r))}{\max_{p,q}L((\psi^{(l)},\dots,\psi^{(1)}), (\mathbf{u}_p\otimes \mathbf{v}_q))} = \begin{cases}
    1, & \mathrm{if} \lambda^\mathbf{W}_l=\lambda^\mathbf{W}_1 \mathrm{and} \lambda^\mathbf{A}_r=\lambda^\mathbf{A}_{1}\\ 0, & \mathrm{otherwise}
    \end{cases}
    $$
\end{proposition}

%remark: the norm of each subspace is precisely given by $L_i(x/||x||) = l^kl^k/l_1l_1$
%remark: Each vector in T_1 is constant across each column.

Note, that this analysis does not use anything related to smoothing. Over-smoothing is merely a consequence because the subspace corresponding to $\lambda_1^\mathbf{W}$ and $\lambda_1^\mathbf{A}$ is spanned by a basis vector with the lowest frequency of the graph laplacian with different scalar multiplicators for different column vectors of $\mathbf{X}$.
As previously shown for this simplified case by Di Giovanni et al.~\cite{di2022graph}, a consequence of this is that the Dirichlet energy $E$ of the normalized node state will converge to zero, for we provide a simplified proof using our new findings:

\begin{proposition}
Let $\mathbf{A}\in\mathbb{R}^{n\times n}$ be the symmetrically normalized adjacency matrix and $\mathbf{W}\in\mathbb{R}^{d\times d}$ be any symmetric matrix. Then, $$\lim_{l\to\infty}E(\frac{\mathbf{X}^{(l)}}{||\mathbf{X}^{(l)}||}) = \mathbf{0}$$
\end{proposition}

As described by Di Giovanni et al.~\cite{di2022graph}, using a residual connection $\mathbf{X}^{(l+1)} = \mathbf{X}^{(l)} + \mathbf{AX}^{(l)}\mathbf{W}$ can prevent over-smoothing depending on the spectrum of $\mathbf{W}$ and instead be dominated by the highest frequency of the graph laplacian. As we show next, this is only the case because a different subspace dominates the representation, but the underlying cause and issue of losing the information present in all other subspaces still persists.

\begin{proposition}
    Using a residual update function, the growth of each subspace is given by $$L_{l,r}(\mathbf{X}^{(l)} + \mathbf{AX}^{(l)}\mathbf{W}) = (\lambda_l^\mathbf{W}\lambda_r^\mathbf{A} + 1)L_{l,r}(\mathbf{X}^{(l)})$$ 
\end{proposition}

When $\lambda_l^\mathbf{W}$ is negative, the residual connection reduces the growth of subspaces that correspond to positive eigenvalues of $\mathbf{A}$ because then $(\lambda^{\mathbf{W}}_l\lambda^\mathbf{A}_r + 1) < \lambda^\mathbf{W}_l\lambda^\mathbf{A}_r$, while also amplifying the growth of subspaces with negative eigenvalues of $\mathbf{A}$. So when $\lambda^\mathbf{W}_1\lambda_1^\mathbf{A} > \lambda^\mathbf{W}_1\lambda_1^\mathbf{A}$, a subspace using the highest frequency dominates the result.
While we find these cases useful for getting an intuition, we now proceed with more general cases. 

%So we are examining how we can achieve that the limit distribution is more than a small subspace.



==> chapters/time_homogeneous.tex <==
%\subsubsection{Time homogeneous case}
%delete
%As each matrix does have $n$ eigenvalues over the field of complex numbers, we will use these to form our subspaces. We also know that for each complex eigenvalue $\lambda_r\in\mathbb{C}$ with eigenvector $\mathbf{x}_r\in\mathbb{C}^{n}$, its complex conjugate $\bar{\lambda}_r\in\mathbb{C}$ is also an eigenvalue with corresponding eigenvector $\bar{\mathbf{x}}_r\in\mathbb{C}^{n}$. Further, the conjugate pairs $\mathbf{x}_r$ and $\bar{\mathbf{x}}_r$ together span a 2-dimensional subspace in $\mathbb{R}$ with basis vectors $Re(\mathbf{x}_r)\in\mathbb{R}^{n\times n}$ and $Im(\mathbf{x}_r)\in\mathbb{R}^{n\times n}$. Therefore, we use this 2-dimensional subspace $\mathbf{V}_i\in\mathbb{R}^{n\times 2}$ in the case of pairs of complex eigenvalues and a 1-dimensional $\mathbf{V}_j\in\mathbb{R}^{n\times 1}$ subspace in the case of real eigenvalues as before.
%We define $\mathbf{V}$ to be the matrix that has all $\mathbf{V}_i$ and $\mathbf{V}_j$ stacked as columns. 
%As before, we combine these with the full $d$-dimensional basis $\mathbf{U}\in\mathbb{R}^{d\times d}$ to form a $(2\cdot d)$-dimensional basis $(\mathbf{U}\otimes \mathbf{V}_i)\in\mathbb{R}^{nd\times 2d}$ corresponding to the complex eigenvalues and $d$-dimensional basis $(\mathbf{U}\otimes \mathbf{V}_j)\in\mathbb{R}^{nd\times d}$ corresponding to the real eigenvalues and the subspace spanned by these basis vectors as $\mathcal{T}_i = span(\mathbf{U}\otimes \mathbf{V}_i)$. We further denote the magnitude of the corresponding eigenvalues of $\mathbf{V}_i$ with $|\lambda^\mathbf{A}_i|$ as both eigenvalues of $\mathbf{x}$ and $\bar{\mathbf{x}}$ have the same magnitude.

%\begin{lemma}
%$\mathcal{T}_i$ is invariant under multiplication with $\mathbf{A}$ and $\mathbf{W}$. All subspaces are linearly independent.
%\end{lemma}

%merge together with w
%We also know from the Perron-Frobenius Theorem~\cite{} that for a non-negative real matrix the maximum eigenvalue is real and all other eigenvalues are smaller in absolute value. Therefore, we can again show that all subspaces that do not correspond to the maximum eigenvalue of $\mathbf{A}$ shrink while this one subspace converge to $L = 1$, which we formally show in the following theorem:

%\begin{theorem}
%Let $\mathbf{U}\in\mathbb{R}^{d\times d}$ be any full rank matrix, $\mathbf{V}\in\mathbb{R}^{n\times n}$ as defined above, and $\mathbf{c}_0$ the solution to $(\mathbf{U}\otimes V)\mathbf{c}_0=vec(\mathbf{x}_0)$. Then,
%\begin{equation*}
%    \lim_{k\to\infty}\frac{L_{i}(\mathbf{X}^{(l)},\mathbf{c}_0)}{max_{p}L_{p}(\mathbf{X}^{(l)}, \mathbf{c}_0)} = \begin{cases}
%    1, & \mathrm{if} \, |\lambda^\mathbf{A}_r|=|\lambda^\mathbf{A}_{1}|\\ 0, & \mathrm{otherwise}
%    \end{cases}
%\end{equation*}
%\end{theorem}

%\subsubsection{Time inhomogeneous case}
%typically the aggregation depends on the updated node states, that can change which nodes have , we consider the mean as a special case with .
